Fusing finetuned models for better pretraining

Pretrained models are the standard starting point for training. This approach consistently outperforms the use of a random initialization. However, pretraining is a costly endeavour that few can undertake. In this paper, we create better base models at hardly any cost, by fusing multiple existing fine tuned models into one. Specifically, we fuse by averaging the weights of these models. We show that the fused model results surpass the pretrained model ones. We also show that fusing is often better than intertraining. We find that fusing is less dependent on the target task. Furthermore, weight decay nullifies intertraining effects but not those of fusing.

==> hf_models.tex <==
We found 92 T5-small models that were not translation models or trained for another language (programmatic or natural) in the \href{https://huggingface.co/models}{HuggingFace hub}. Out of these, 14 mismatched in dimensions, after altering some layers in the architecture and were discarded completely. So were 2 models trained on JAX and 30 models that failed to load. Out of the 46 models left (full list in App.~\ref{ap:sec:hf_models}), we identified 26 as tuned for summarization by containing one of the following strings: "sum", "cnn", "dm", "headline", "bbc", "giga". Out of which 17 were presumably tuned on the large dataset XSUM \cite{Narayan2018DontGM}. Similarly, 8 models were tuned for question answering as shown by the strings: "qa", "question", "CANARD", "Qu", "qu".
We created several combinations of models to see whether those, despite being unrelated to the tasks tested (general text classification tasks) could help. The fuse model groups were all (Fuse HF), summarization models, QA models, and all models but just one (last chronologically) XSUM model.


aseda/t5-small-finetuned-xsum,
furyhawk/t5-small-finetuned-bbc-headline,
gniemiec/t5-small-finetuned-xsum,
Teepika/t5-small-finetuned-xsum-proplus,
Frederick0291/t5-small-finetuned-billsum,
aristotletan/t5-small-finetuned-xsum,
furyhawk/t5-small-finetuned-bbc,
gwynethfae/t5-small-finetuned-xsum,
mengsay/t5-small-finetuned-gigaword,
usami/t5-small-finetuned-xsum,
Teepika/t5-small-finetuned-xsum-gcloud1,
erwanlc/t5-coktails\_recipe-small,
mrm8488/t5-small-finetuned-boolq,
bochaowei/t5-small-finetuned-xsum-wei1,
bochaowei/t5-small-finetuned-cnn-wei0,
bochaowei/t5-small-finetuned-xsum-wei1,
Frederick0291/t5-small-finetuned-xsum,
bochaowei/t5-small-finetuned-xsum-wei0,
Frederick0291/t5-small-finetuned-xsum,
mrm8488/t5-small-finetuned-quora-for-paraphrasing,
allenai/unifiedqa-t5-small,
allenai/t5-small-squad2-question-generation,
mrm8488/t5-small-finetuned-wikiSQL,
Unbabel/gec-t5\_small,
pki/t5-small-finetuned\_xsum,
hetpandya/t5-small-tapaco,
allenai/t5-small-next-word-generator-qoogle,
mrm8488/t5-small-finetuned-emotion,
allenai/t5-small-squad2-next-word-generator-squad,
bochaowei/t5-small-finetuned-cnn-wei1,
mrm8488/t5-small-finetuned-imdb-sentiment,
RenZHU/t5-small-finetuned-xsum,
stevhliu/t5-small-finetuned-billsum-ca\_test,
hetpandya/t5-small-quora,
mrm8488/t5-small-finetuned-common\_gen,
bhuvaneswari/t5-small-text\_summarization,
allenai/t5-small-squad11,
danyaljj/unifiedqa-t5-small,
khanglam7012/t5-small,
airKlizz/t5-small-multi-combine-wiki-news,
mrm8488/t5-small-finetuned-squadv2,
jazzisfuture/new\_summary\_t5\_small,
bhuvaneswari/t5-small-finetuned-xsum,
nouamanetazi/cover-letter-t5-small,
fadhilarkan/t5-small-finetuned-xsum-2,
RenZHU/t5-small-finetuned-xsum-original

==> old.tex <==
\section{Results old}
In this section, we follow our hypothesis from large to small. First, we show in Fig.~\ref{fig:glue} that, in general, fusing is helpful. Fusing the unrelated tasks in GLUE and SUPER-GLUE helps on other GLUE and SUPER-GLUE. Fusing is better than finetuning T5 in a ratio of 9:4 and than inter-training 9:4. This is surprising, as in the literature, the models of most intermediate tasks we fused upon are not beneficial for most tasks. This shows careful model choice might not be as crucial for fusing as it is for intertraining.

However, we do see that when restricting ourselves to a set of models trained on similar tasks (Fig.~\ref{fig:nli}) or on the same domain (Fig.~\ref{fig:tweet_eval}) results are strong. In this context, it is interesting to note that among the NLI datasets one (WNLI) is in the same task format but is not actually dealing with inference, but gender. This dataset is also the only one not to benefit from fusing the NLI datasets.



HellaSwag has proven a very strong baseline (Fig.~\ref{fig:hella}). However, while rerunning the experiments with a different seed (Fig.~\ref{fig:hella_seed0}), it is less so and fuse is better. We will rerun with several seeds to get a clearer picture.

We find (App.~\ref{ap:sec:twitter_long_short}) fusing models that trained on more data is generally better. However, fusing several relevant models, despite some of them trained on small sized datasets, does seem to be better.

Topical results are inconclusive (Fig.~\ref{fig:topic})
\subsection{Uncontrolled experiments}\label{sec:uncontrolled}
We compare various fused models based on models publicly available at the time of writing. We find in both seeds the training outperforms the intermediate task baselines. Both summarization and QA models are fused well as a pretraining model  (Fig.~\ref{fig:hf}) outperforming both those baselines and more often than not the train (5:8 and 4:8 respectively) and other fused models. This might suggest fusing similar models brings more of their learning forward and prevents interference, this will be checked in future work. Notably, fusing all models (except the repeating XSUMs) performs quite well too, and if nothing else is not worse than the pretraining and is better than the intermediate tasks HellaSwag and MNLI.

Last we consider the realistic case where one has some task and many unknown models. We train on 411 finetuned models finetuned on the above datasets during our initial trials with different variations (learning rates, limited amount of data, random seeds, datasets etc.). Evidently, combining them is also beneficial, despite the uncontrolled set of models. While the difference is not large, it still outperform finetuning T5 (9:3) and also fusing models tuned on the full datasets of the general case (8:3) (Fig.~\ref{fig:glue}).

\section{Related work}
\section{Next experiments}
\begin{itemize}
\item rearrange twitter data
\item report how many times in exp fuse is better than continue and from train
\item get any good results where easiest to get:
\begin{itemize}
    \item improve overleaf
    \item sentiment (/topic) - run and try to change to make it better - elad 
    \item try large vs. small subsets - tweet-eval (and weight by amount of data for training) - elad
    \item few shot glue - Leshem
    \item run T5 on GLUE without different labels and dataset-names(post-input) - Leshem
    \item run on a larger T5-1.1 (base) - Leshem
    \item fuse existing models from HF hub - Leshem
    \item hella on twitter/hellaswag
    \item does fusing on glue better or worse for Twitter/nli?
    \item fuse on cosmosQA with hella and mnli %({mamlong34/t5_small_cosmos_qa}) 
    as it is another dataset that is known to be good intermediate (the last is comonsense QA)
    \item chunks with large pretraining and small finetuning (maybe need to change runnable so data won't overlap)
    \item fisher
    \item weighted by something (norms, data amount?)

\end{itemize}
\item Show properties of where it helps
\begin{itemize}
    \item How much fusing more finetuned models helps  (Take it where it helped and reduce the number of fused models? maybe also on chunks)
    \item Which dataset helps more (where most helped, maybe NLI)
    \item How more helpful is it when finetuning is scarce?
    \item Does combining the same dataset multiple times ruin? help? doesn't matter?
    \item the effect of many models for fusing vs less models (either trained on the same total data or of repetitions where models get the same data but are still fused)
\end{itemize}
\item Try non-leave one out
\end{itemize}



\begin{figure}[tbp]
\includegraphics[width=8cm]{nli.png}
\caption{Fusing improves over both pretrained model and over using the model trained on the largest dataset as pretrained. NLI results with two seeds. 0 is regular training 1 is continue over the largest dataset and 2 is fusing all models not trained on the finetuning dataset.}
\label{fig:times}
% \vspace{-0.3cm}
\end{figure}
% Entries for the entire Anthology, followed by custom entries

